ChatEL: Entity Linking with Chatbots

Entity Linking (EL) is an essential and challenging task in natural language processing that seeks to link some text representing an entity within a document or sentence with its corresponding entry in a dictionary or knowledge base. Most existing approaches focus on creating elaborate contextual models that look for clues the words surrounding the entity-text to help solve the linking problem. Although these fine-tuned language models tend to work, they can be unwieldy, difficult to train, and do not transfer well to other domains. Fortunately, Large Language Models (LLMs) like GPT provide a highly-advanced solution to the problems inherent in EL models, but simply naive prompts to LLMs do not work well. In the present work, we define ChatEL, which is a three-step framework to prompt LLMs to return accurate results. Overall the ChatEL framework improves the average F1 performance across 10 datasets by more than 2%. Finally, a thorough error analysis shows many instances with the ground truth labels were actually incorrect, and the labels predicted by ChatEL were actually correct. This indicates that the quantitative results presented in this paper may be a conservative estimate of the actual performance. All data and code are available as an open-source package on GitHub at https://github.com/yifding/In_Context_EL.

==> table/error_case_study.tex <==
%\resizebox{\textwidth}{!}{%
%{
\begin{tabular}{ccccc}
\toprule
Dataset & Degree of Error & Ground Truth & Prediction & Reason Analysis \\
ACE04	&high	&Ministry of Defense (Iran)	&Ministry of Defense (Japan)	&2nd prompt  \\
ACE04	&high	&Florida	&Florida Legislature	&2nd prompt \\
ACE04	&low	&President of Egypt	&President	&2nd prompt \\
ACE04	&low	&Gaza City	&Gaza Strip	&1st prompt \\
ACE04	&low	&Volvo	&Volvo Cars	&2nd prompt    \\
KORE	&low	&First Ladies of Argentina	&First Lady	&1st prompt \\
KORE	&high	&Justin Bieber	&Justin I	&1st prompt \\
KORE	&high	&Lady Gaga	&Gwen Stefani	&2nd prompt \\
KORE	&high	&Desire (Bob Dylan album)	&Desire	&post-processing \\
KORE	&high	&Paul Allen	&NULL	&1st prompt \\
AQU	&high	&Cancer	&Lung Cancer	&2nd prompt \\
AQU	&high	&Tissue (biology)	&Facial tissue	&2nd prompt \\
AQU	&high	&Radiation	&Ionizing Radiation	&2nd prompt \\
AQU	&high	&Federation	&Malaysian Roads System	&1st prompt \\
AQU	&high	&Federated State	&States of India	&2nd prompt \\
CWEB	&high	&Head	&Head (company)	&1st prompt \\
CWEB	&-	&Hillsborough County, Florida	&Hillsborough, North Carolina	&GT is incorrect \\
CWEB	&low	&Lake Wylie	&Lake Wylie, South Carolina	&2nd prompt \\
CWEB	&-	&Australia Cricket Team	&Australia	&GT is incorrect \\
CWEB	&high	&England Cricket Board	&European Central Bank	&2nd prompt \\
MSN	&high	&Associated Press	&Arnold Ap	&2nd prompt \\
MSN	&-	&New York City	&New York	&GT is incorrect \\
MSN	&-	&University of Alabama	&Alabama Crimson Tide football	&GT is incorrect \\
MSN	&high	&Sago Mine Disaster	&Sago, West Virginia	&1st prompt \\
MSN	&high	&World Trade Center	&Collapse of the World Trade Center	&2nd prompt \\
OKE15	&-	&Fellow	&Research Fellow	&GT is incorrect \\
OKE15	&low	&Cambridge	&University of Cambridge	&1st prompt \\
OKE15	&-	&Principal (academia)	&Head teacher	&GT is incorrect \\
OKE15	&low	&Faculty (academic staff)	&Professor	&1st prompt \\
OKE15	&-	&Officer	&Officer (armed forces)	&GT is incorrect \\
OKE16	&-	&Director (business)	&Executive director	&GT is incorrect \\
OKE16	&-	&Germany	&Nazi Germany	&GT is incorrect \\
OKE16	&-	&Czechs	&Czech Republic	&GT is incorrect \\
OKE16	&high	&Salvatore Quasimodo	&Quasimodo	&1st prompt \\
OKE16	&-	&Sorbonne	&University of Paris	&GT is incorrect \\
REU	&high	&Oregon	&Ore	&post-processing \\
REU	&-	&Georgia Power	&Georgia (U.S. state)	&GT is incorrect \\
REU	&low	&Lloyds Bank of Canada	&Lloyds Bank	&2nd prompt \\
REU	&high	&Continental Bank of Canada	&Continental philosophy	&1st prompt \\
REU	&high	&J. P. Morgan	&Morgan Motor Company	&1st prompt \\
RSS	&-	&Steve Jobs	&Apple Inc.	&GT is incorrect \\
RSS	&low	&Pro Bowl	&Super Bowl	&2nd prompt \\
RSS	&high	&Pro Bowl	&Bowl Game	&2nd prompt \\
RSS	&-	&Eric Kearney	&Cincinnati	&GT is incorrect \\
RSS	&high	&Cleveland Browns	&Cleveland	&2nd prompt \\
WIKI &low	&Croatia Speedway Team	&Croatia	&2nd prompt \\
WIKI	&low	&Little Caesars Pizza Bowl	&2009 Little Caesars Pizza Bowl	&prediction is better \\
WIKI	&low	&Ohio Bobcats football	&Ohio Bobcats	&2nd prompt \\
WIKI	&low	&Leasehold estate	&Renting	& 1st prompt \\
WIKI	&low	&Real Estate Pricing	&House Price Index	&2nd prompt \\

\bottomrule
\end{tabular}
%}
%}


